Towards Universal Mesh Movement Networks

Solving complex Partial Differential Equations (PDEs) accurately and efficiently is an essential and challenging problem in all scientific and engineering disciplines. Mesh movement methods provide the capability to improve the accuracy of the numerical solution without increasing the overall mesh degree of freedom count. Conventional sophisticated mesh movement methods are extremely expensive and struggle to handle scenarios with complex boundary geometries. However, existing learning-based methods require re-training from scratch given a different PDE type or boundary geometry, which limits their applicability, and also often suffer from robustness issues in the form of inverted elements. In this paper, we introduce the Universal Mesh Movement Network (UM2N), which -- once trained -- can be applied in a non-intrusive, zero-shot manner to move meshes with different size distributions and structures, for solvers applicable to different PDE types and boundary geometries. UM2N consists of a Graph Transformer (GT) encoder for extracting features and a Graph Attention Network (GAT) based decoder for moving the mesh. We evaluate our method on advection and Navier-Stokes based examples, as well as a real-world tsunami simulation case. Our method outperforms existing learning-based mesh movement methods in terms of the benchmarks described above. In comparison to the conventional sophisticated Monge-Amp\`ere PDE-solver based method, our approach not only significantly accelerates mesh movement, but also proves effective in scenarios where the conventional method fails. Our project page is at https://erizmr.github.io/UM2N/.

==> sections/rebuttal.tex <==
\appendix
\setcounter{section}{0}

% \section*{Appendix}

\setcounter{section}{0}
\setcounter{figure}{0}
\makeatletter 
\renewcommand{\thefigure}{R\arabic{figure}}% Figure counter representation
\renewcommand{\theHfigure}{R\arabic{figure}}% Hyperref figure hyperlink hook
\renewcommand{\thetable}{R\arabic{table}}
\renewcommand{\theHtable}{R\arabic{table}}

\makeatother
\setcounter{table}{0}
\setcounter{equation}{0}
\renewcommand{\theequation}{R\arabic{equation}}


\begin{table}%{0.8\textwidth}
\vspace{-4mm}
\caption{Ablation Study for components of network architecture.}% 
\centering
% \vspace{-2mm}
\resizebox{0.6\textwidth}{!}{
 \begin{tabular}{lr}
  \toprule[1pt]
  \midrule
  & Swirl \\
  % \cmidrule(rrr){2-3}
  % \cmidrule(rr){5-6}
  % \cmidrule(r){7}
  Method & ER $\uparrow$ (\%)   \\
  \midrule
  UM2N-w/o-Decoder  & 10.68      \\
  UM2N-w/o-GT &  12.35    \\
  \textbf{UM2N (Ours)} & 35.93   \\
  MA (reference) & 37.43   \\
  \midrule
  \bottomrule[1pt]
 \end{tabular}
}
\vspace{-4mm}
\label{tab:ablation_study}
\end{table}


\begin{table}%{0.8\textwidth}
\vspace{-4mm}
\caption{Measure between model output mesh and MA reference.}% 
\centering
% \vspace{-2mm}
\resizebox{0.8\textwidth}{!}{
 \begin{tabular}{lrrr}
  \toprule[1pt]
  \midrule
  & Train & Test & Reduce \\
  % \cmidrule(rrr){2-3}
  % \cmidrule(rr){5-6}
  % \cmidrule(r){7}
  Method & Start / End  & Start / End & Ratio (Train) \\ 
  \midrule
  Element volume loss  & 66.09/17.40 & 60.11/17.54 &  73.6 \% \\
  Chamfer distance &  3.40/1.43 &  2.46/1.52 &   57.9 \% \\
  \midrule
  \bottomrule[1pt]
 \end{tabular}
}
\vspace{-4mm}
\label{tab:ablation_study}
\end{table}



\begin{table}%{0.8\textwidth}
\vspace{-4mm}
\caption{Measure between model output mesh and MA reference.}% 
\centering
% \vspace{-2mm}
\resizebox{0.8\textwidth}{!}{
 \begin{tabular}{lrr}
  \toprule[1pt]
  \midrule
  % \cmidrule(rrr){2-3}
  % \cmidrule(rr){5-6}
  % \cmidrule(r){7}

  & M2N & UM2N \\
  % \cmidrule(rrr){2-3}
  % \cmidrule(rr){5-6}
  % \cmidrule(r){7}
  Property & ER $\uparrow$ (\%) & ER $\uparrow$ (\%)   \\
  % Error Reduction & M2N  & UM2N  \\ 
  \midrule
   Vorticity &  \textbf{27.43} \% & 10.22 \%  \\
  \midrule
  \bottomrule[1pt]
 \end{tabular}
}
\vspace{-4mm}
\label{tab:ablation_study}
\end{table}

